A self-consistent spin-diffusion model for micromagnetics

We propose a three-dimensional micromagnetic model that dynamically solves the Landau-Lifshitz-Gilbert equation coupled to the full spin-diffusion equation. In contrast to previous methods, we solve for the magnetization dynamics and the electric potential in a self-consistent fashion. This treatment allows for an accurate description of magnetization dependent resistance changes. Moreover, the presented algorithm describes both spin accumulation due to smooth magnetization transitions and due to material interfaces as in multilayer structures. The model and its finite-element implementation are validated by current driven motion of a magnetic vortex structure. In a second experiment, the resistivity of a magnetic multilayer structure in dependence of the tilting angle of the magnetization in the different layers is investigated. Both examples show good agreement with reference simulations and experiments respectively.

==> translator-language-mappings.tex <==
% Copyright 2007 by Till Tantau
% Copyright 2010 by Vedran Mileti\'c
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the documentation file for more details.

\def\trans@use@and@alias#1#2{%
  \uselanguage{#2}%
  \languagealias{#1}{#2}%
}

\DeclareOption{acadian}        {\trans@use@and@alias{french}    {Acadian,French}}
\DeclareOption{afrikaans}      {\trans@use@and@alias{afrikaans} {Afrikaans,Dutch}}
\DeclareOption{american}       {\trans@use@and@alias{american}  {AmericanEnglish,English}}
\DeclareOption{austrian}       {\trans@use@and@alias{austrian}  {Austrian1997,Austrian,German1997,German}}
\DeclareOption{bahasa}         {\trans@use@and@alias{bahasa}    {Bahasa}}
\DeclareOption{basque}         {\trans@use@and@alias{basque}    {Basque}}
\DeclareOption{brazil}         {\trans@use@and@alias{brazil}    {Brazilian,Portuguese}}
\DeclareOption{brazilian}      {\trans@use@and@alias{brazilian} {Brazilian,Portuguese}}
\DeclareOption{breton}         {\trans@use@and@alias{breton}    {Breton}}
\DeclareOption{british}        {\trans@use@and@alias{british}   {BritishEnglish,English}}
\DeclareOption{bulgarian}      {\trans@use@and@alias{bulgarian} {Bulgarian}}
\DeclareOption{canadian}       {\trans@use@and@alias{canadian}  {Canadian,English}}
\DeclareOption{canadien}       {\trans@use@and@alias{canadien}  {Canadien,French}}
\DeclareOption{catalan}        {\trans@use@and@alias{catalan}   {Catalan}}
\DeclareOption{croatian}       {\trans@use@and@alias{croatian}  {Croatian}}
\DeclareOption{czech}          {\trans@use@and@alias{czech}     {Czech}}
\DeclareOption{danish}         {\trans@use@and@alias{danish}    {Danish}}
\DeclareOption{dutch}          {\trans@use@and@alias{dutch}     {Dutch}}
\DeclareOption{english}        {\trans@use@and@alias{english}   {English}}
\DeclareOption{esperanto}      {\trans@use@and@alias{esperaton} {Esperanto}}
\DeclareOption{estonian}       {\trans@use@and@alias{estonian}  {Estonian}}
\DeclareOption{finnish}        {\trans@use@and@alias{finnish}   {Finnish}}
\DeclareOption{francais}       {\trans@use@and@alias{french}    {French}}
\DeclareOption{frenchb}        {\trans@use@and@alias{french}    {French}}
\DeclareOption{french}         {\trans@use@and@alias{french}    {French}}
\DeclareOption{galician}       {\trans@use@and@alias{galician}  {Galician}}
\DeclareOption{german}         {\trans@use@and@alias{german}    {German1997,German}}
\DeclareOption{germanb}        {\trans@use@and@alias{german}    {German1997,German}}
\DeclareOption{greek}          {\trans@use@and@alias{greek}     {Greek}}
\DeclareOption{polutonikogreek}{\trans@use@and@alias{greek}     {Polutoniko,Greek}}
\DeclareOption{hebrew}         {\trans@use@and@alias{hebrew}    {Hebrew}}
\DeclareOption{hungarian}      {\trans@use@and@alias{hungarian} {Hungarian}}
\DeclareOption{icelandic}      {\trans@use@and@alias{icelandic} {Icelandic}}
\DeclareOption{irish}          {\trans@use@and@alias{irish}     {Irish}}
\DeclareOption{italian}        {\trans@use@and@alias{italian}   {Italian}}
\DeclareOption{latin}          {\trans@use@and@alias{latin}     {Latin}}
\DeclareOption{lowersorbian}   {\trans@use@and@alias{lsorbian}  {LowerSorbian,Sorbian}}
\DeclareOption{magyar}         {\trans@use@and@alias{magyar}    {Magyar}}
\DeclareOption{naustrian}      {\trans@use@and@alias{naustrian} {Austrian,German}}
\DeclareOption{ngerman}        {\trans@use@and@alias{ngerman}   {German}}
\DeclareOption{norsk}          {\trans@use@and@alias{norsk}     {Norsk}}
\DeclareOption{samin}          {\trans@use@and@alias{samin}     {Samin}}
\DeclareOption{nynorsk}        {\trans@use@and@alias{nynorsk}   {Nynorsk,Norsk}}
\DeclareOption{polish}         {\trans@use@and@alias{polish}    {Polish}}
\DeclareOption{portuges}       {\trans@use@and@alias{portuges}  {Portuguese}}
\DeclareOption{portuguese}     {\trans@use@and@alias{portuguese}{portuguese}}
\DeclareOption{romanian}       {\trans@use@and@alias{romanian}  {Romanian}}
\DeclareOption{russian}        {\trans@use@and@alias{russian}   {Russian}}
\DeclareOption{scottish}       {\trans@use@and@alias{scottish}  {Scottish}}
\DeclareOption{serbian}        {\trans@use@and@alias{serbian}   {Serbian}}
\DeclareOption{slovak}         {\trans@use@and@alias{slovak}    {Slovak}}
\DeclareOption{slovene}        {\trans@use@and@alias{slovene}   {Slovene}}
\DeclareOption{spanish}        {\trans@use@and@alias{spanish}   {Spanish}}
\DeclareOption{swedish}        {\trans@use@and@alias{swedish}   {Swedish}}
\DeclareOption{turkish}        {\trans@use@and@alias{turkish}   {Turkish}}
\DeclareOption{ukrainian}      {\trans@use@and@alias{ukrainian} {Ukrainian}}
\DeclareOption{uppersorbian}   {\trans@use@and@alias{usorbian}  {UpperSorbian,Sorbian}}
\DeclareOption{welsh}          {\trans@use@and@alias{welsh}     {Welsh}}
\DeclareOption{UKenglish}      {\trans@use@and@alias{UKenglish} {BritishEnglish,English}}
\DeclareOption{USenglish}      {\trans@use@and@alias{USenglish} {AmericanEnglish,English}}
\ProcessOptions*

